Learning Hierarchy Aware Features for Reducing Mistake Severity

Label hierarchies are often available apriori as part of biological taxonomy or language datasets WordNet. Several works exploit these to learn hierarchy aware features in order to improve the classifier to make semantically meaningful mistakes while maintaining or reducing the overall error. In this paper, we propose a novel approach for learning Hierarchy Aware Features (HAF) that leverages classifiers at each level of the hierarchy that are constrained to generate predictions consistent with the label hierarchy. The classifiers are trained by minimizing a Jensen-Shannon Divergence with target soft labels obtained from the fine-grained classifiers. Additionally, we employ a simple geometric loss that constrains the feature space geometry to capture the semantic structure of the label space. HAF is a training time approach that improves the mistakes while maintaining top-1 error, thereby, addressing the problem of cross-entropy loss that treats all mistakes as equal. We evaluate HAF on three hierarchical datasets and achieve state-of-the-art results on the iNaturalist-19 and CIFAR-100 datasets. The source code is available at https://github.com/07Agarg/HAF

==> Sections/approach.tex <==
% \subsection{Notations}

% For a given hierarchy tree with $H+1$ number of hierarchical levels, $K^h$ be the number of classes at the $h$-th level of the hierarchy, where $h=1$ corresponds to coarsest ($h=0$ is the root node) and $h=H$ is the finest-level. \ours leverages hierarchical classifiers at different levels of hierarchy. Let $\cal{F}(.)$ be the feature extractor and ${\cal{G}}^h(.)$ %${\cal{G}}^1(.)$, ${\cal{G}}^2(.)$ $\ldots$ ${\cal{G}}^H(.)$ 
% be different hierarchical classifiers with parameters $\theta^h$. %$\theta_1, \theta_2 \ldots \theta_H$ respectively. 

% Let $\cal{X}$ = $\{ x_i, y_i^h \}$ be the set of images and their labels at level $h$. Let $ p^h(\hat{y_i}^h|x_i;\theta^h) $ = ${\cal{G}}^h(F(x_i))$ refers to the predicted probability of image $x_i$ from the model from $h$-level hierarchical classifier.  % where $h$ $\in$ [$1, 2, \ldots H$].

% \subsection{\JSD}

% In HAF, we enforce consistency across the hierarchical classifiers. We minimize the Jensen-Shannon (JS) Divergence between the predicted probability of a coarse class and the  approximated probability distribution using its component distributions.

% Let $\widehat{p}^h(\hat{y_i}^h|x_i;\theta^h)$ be the approximated probability of a class at a coarse-level $h$ using mixture distributions of its components at level $h+1$. Then, the approximated probability of a coarse class at level $h$ is sum of probabilities of its component sub-classes following the law of total probability. Let `$A$' be a coarse class at level $h$ and $A_1$, $A_2$, $\ldots$ $A_k$ be $k$ sub-classes of coarse class $A$.  

% % `$A_1$' and `$A_2$' be its sub-classes. 

% \begin{equation}
% \widehat{p}^h(\hat{y_i}=A|x_i;\theta^h) = \sum_{c=1}^{k} p^{(h+1)}(\hat{y_i}=A_c|x_i;\theta^{h+1})
% %p^{(h+1)}(\hat{y_i}=A_1|x_i;\theta_{h+1}) + p^{(h+1)}(\hat{y_i}=A_2|x_i;\theta_{h+1})
% \end{equation}

% Jensen-Shannon (JS) divergence is minimized between predicted probability from $h$-level classifier $ p^h(\hat{y_i}^h|x_i;\theta_h) $ and the approximated probability of the class from at coarse-level $\widehat{p}^h(\hat{y_i}^h|x_i;\theta_h)$. For simplicity, we use $p^h$ to refer to $ p^h(\hat{y_i}^h|x_i;\theta_h) $ and $\hat{p}^h$ for $\widehat{p}^h(\hat{y_i}^h|x_i;\theta_h)$. Jensen-Shannon (JS) divergence loss is computed using the following:

% \begin{gather}
% \text{JS}_{h, h+1}(p^h ; \hat{p}^h) = \frac{1}{2}(\text{KL}(p^h || m) + \text{KL}(\hat{p}^h || m))
% \end{gather}
% where $m$ = $\frac{1}{2}(p^h + \widehat{p}^h)$ and KL refers to Kullback-Leibler divergence. \\

% We compute \JSD pairwise across the levels. The total \JSD is the following: 

% \begin{gather}
% \text{JS}_{total} = \sum_{h=1}^{h=H-1}{\text{JS}_{h, h+1}(p^h ; \hat{p}^h)}
% \end{gather}

% \subsection{\weightconst}
% The weight vectors of different classifiers learned in a hierarchy-aware feature space should be aligned. The weight vector of a coarse-class should be aligned with the linear combination of the weight vectors of its fine-grained classes. We first normalize the weight vectors of all the classes across all the classifiers before applying softmax at the output. For a class $c$ at any level $h$, the l2-normalized weight is given by:  
%  \begin{gather}
%     W_c^h = \frac{W_c^h}{||W_c^h||_2}
% \end{gather}
% We re-normalize all the weight vectors to lie on a normalized hypersphere, 
% % Adding weight constraints: \\
% %     First L2-Normalize weights:
   
%     % Softmax Loss: 
%     % \begin{gather}
%     %     \text{minimize} \frac{-1}{M} \sum_{i=1}^{N}\text{log} (\frac{{e^{W_{ci}^{h^T}} f(xi) + b_{ci}^h}}{\sum_{j=1}^{C} e^{W_{ci}^{h^T} f(xi) + b_{ci}^h}})
%     % \end{gather}
%     % Again L2-normalize weights;
%     % \begin{gather}
%     %     W_c^h = \frac{W_c^h}{||W_c^h||_2}
%     % \end{gather}
%     % Convex combination (summation) of weights of sub-classes of a super-class (L2-normalized vectors) should be aligned to L2-normalized weight vector of that coarse class. 
%     We denote the weight vector of coarse class $A$ at level $h$ by $W_A^h$. Let $c$ $\in\{1, 2, \ldots k\}$ represents indices of the sub-classes at level $h+1$ belonging to the coarse-class $A$ at level $h$. We hypothesize that the convex combination of weight vectors of sub-classes of a super class should be aligned with the weight vector of its coarse class. For simplicity, we use the summation of the weight vectors of the sub-classes to represent the weight vector of the super-class. The approximated weight vector using summation is thus given by:
%     \begin{gather}
%         \hat{W_A^h} = \sum_{c=1}^{k}W_c^{h+1}
%     \end{gather}
%     Now, we maximize the cosine similarity between $W_A^h$ and $\hat{W_A^h}$.
%     \begin{gather}
%       L_{sim_h} = \text{cos}(W_A^h, \hat{W_A^h})
%     \end{gather}

% \subsection{\dissimilar}
% The \dissimilar uses dissimilar pairs at coarser-levels. We maximize the Jensen Shannon (JS) divergence between the probability distribution of dissimilar pairs. The pairwise \dissimilar at any level $h$ is given by: 

% \begin{gather}
%     L_{dsim_h} = max(0, m - \text{JS}_h(p ; q))
% \end{gather}

% where $m$ is the margin and $p$ and $q$ are the probability distributions of dissimilar pairs from classifier at level $h$. 

% The total dissimilar loss $L_{dsim}$ is given by: 
% \begin{gather}
%     L_{dsim} = \sum_{h=1}^{h=H-1} L_{dsim_h}
% \end{gather}

% Total loss is thus given by: ???? 

% % Let $H$ be the number of hierarchical levels, $K^i$ be the number of classes at the $i$-th level of the hierarchy, where $i=1$ corresponds to coarsest and $i=H$ is the finest-level. Let $\cal{F}(.)$ be the feature extractor and ${\cal{G}}^1(.)$, ${\cal{G}}^2(.)$, ${\cal{G}}^3(.)$ $\ldots$ ${\cal{G}}^H(.)$ be different hierarchical classifiers. 

% % Let $\cal{X}$ = $\{ x_i, y_i^h \}$ be the set of images and their labels at level $h$ where $h$ $\in$ [$1, 2, \ldots H$]. Let $p^h(\hat{y_i}|x_i;\theta)$ = ${\cal{G}}^h(F(x_i))$ refers to the predicted probability of image $x_i$ from the model $\theta$ from $h$-level hierarchical classifier. 

% %To model the hierarchies in the data, mixture distributions can be one of the possible ways. The finest level of the hierarchy can be considered to be the distribution of the fine-grained classes. Semantically similar classes should follow similar data distribution and therefore, higher levels of hierarchy can be composite of mixture distributions of semantically similar classes. For a super-class $C$ at level $h$ and its sub-classes $c \in C$ at level $h+1$.

% \begin{comment}
% \begin{gather}
% p^h(\hat{y_i}=C|x_i;\theta) = \sum_{c \in C} \pi_i   p^{h+1}(\hat{y_i}=c|x_i;\theta)
% \end{gather}
% where $\Pi_i$ represents the mixing weights. Can be a uniform distribution, or, ... 
% \end{comment}


==> Sections/proposed_approach_with_KD.tex <==
% \subsection{Notation}

Consider a label hierarchy tree with $H+1$ levels, where the root is at level-0, and $h\in[1,\ldots,H]$ denote the hierarchical level with $h\!=\!1$ and $h\!=\!H$ the coarsest and finest levels respectively. We ignore the root node for our purposes as it denotes the universal super-set containing all classes. Let $\cal{X}$ = $\{ \bx_i, y_i^h \vert i=1,\ldots,N \}$ be the set of $N$ images and their respective ground-truth labels at level $h$. We denote the common feature extractor $f_{\phi}(\cdot)$, which is implemented using some backbone neural network and is parameterized by $\phi$. As illustrated in Fig. \ref{fig:proposed_approach}, we use classifiers at each level of the hierarchy in training \ours and denote the level-$h$ classifier as $g^h(\cdot)$ parameterized by the weight matrix $\bW^h$. The resulting prediction probabilities are denoted by $ p^h(\widehat{y}_i^h|\bx_i;\bW^h) = g^h(f_{\phi}(\bx_i))$, where $\widehat{y}_i^h$ is the label predicted for $\bx_i$ by $g^h(\cdot)$ and can take class labels from the set of classes at level-$h$ as $\calC^{h}=\left\{ \bigcup_{i=1}^{|A|} A_i, \bigcup_{i=1}^{|B|} B_i, \bigcup_{i=1}^{|C|} C_i, \ldots\right\}$, where we define the set of classes at level-$(h-1)$ as $\calC^{h-1}=\{A,B,C,\ldots\}$. With a slight abuse of notation, here we use $A$ to denote a super-class label at level-$(h-1)$ and the set of its sub-classes $\{A_1,A_2,\ldots\}$ at level-$h$. % This notation should be sufficient to develop our loss functions, where the terms only rely on consecutive levels of the hierarchy.  

%Let $ p^h(\widehat{y}_i^h|\bx_i;\btheta^h) $ = ${\cal{G}}^h(F(\bx_i))$ refer to the predicted softmax probability distribution from the $h$-level hierarchical classifier. Therefore, $\widehat{y}_i^h$ = $\arg\max_{k\in K^h} p^h(y_i^h=k|x_i;\theta^h)$, where $K^h$ is the set of classes at level-$h$.

%Let $\hat{y_i}^h$ = ${\cal{G}}^h(F(x_i))$ denotes the predicted label and  $ p^h(\hat{y_i}^h|x_i;\ \theta^h) $ refers to its predicted probability from $h$-level hierarchical classifier.  % where $h$ $\in$ [$1, 2, \ldots H$].

\subsection{\CEfinest  ($L_{CE_{fine}}$)} 

We use the ground truth labels only at the finest level of the hierarchy and apply the cross-entropy loss to train the level-$H$ classifier, i.e.,  ${g}^H(\cdot)$. The fine-grained cross-entropy loss for a sample is given by
\begin{gather}
L_{CE_{fine}} = - \sum_{c\in\calC^H} \mathbf{1}\!\left[y_i^H\!=\!c\right]\log \left(p^H(\widehat{y}_i^H\!=\!c|\bx_i;\bW^H)\right)
\label{eqn:cross-entropy}
\end{gather}
where $\mathbf{1}[\cdot]$ serves as an indicator function and takes a value of one when the argument is true, else zero. 

\subsection{\JSD ($L_{shc}$)}
For making better mistakes, we want the classifiers at all levels to use the same feature space and yet make predictions consistent with the label hierarchy. While it is natural to use the cross-entropy loss for training the classifiers at all levels, as noted in \cite{flamingo_2021_Chang} and observed during our initial experiments, this choice of loss compromises the fine-grained accuracy. Instead, we encourage online peer-distillation \cite{zhang_2018_CVPR,zhu_2018_NIPS,chen_2020_AAAI} between the classifiers at different levels. While the fine-grained classifier is trained with the cross-entropy loss ($L_{CE_{fine}}$), the coarse-classifiers learn the relevant information by knowledge transfer from the finer-grained classifiers. Motivated by state-of-the-art methods \cite{zhang_2018_CVPR,chen_2022_CVPR}, we enforce mutual learning between the classifiers, which enables them to teach each other and learn collaboratively. This loss is inspired from the fact that higher predictions of fine-classes should lead to higher predictions of corresponding coarse-classes. Unlike conventional logit-based distillation \cite{44873,zhang_2018_CVPR,zhu_2018_NIPS,chen_2020_AAAI} strategies where the number of classes in each network/classifier is the same, these number of classes of each classifier is different in \ours. Therefore, to enable the distillation between the classifiers at different levels, we use predictions of a coarse classifier $g^{h-1}(\cdot)$ and the \textit{soft-labels} obtained from the next fine-level classifier $g^{h}(\cdot)$. We introduce Jensen-Shannon Divergence (JSD) \cite{fuglede_2004_jensen} as the distillation loss. % between the predictions of a coarse classifier $g^{h-1}(\cdot)$ and the soft labels obtained from the next fine-level classifier $g^h(\cdot)$. % we use the probability distribution of coarse-classifier as is and obtain the soft-labels for fin
% collaboratively, teach each other, mutual learning, online learning, peer learning, logit-based distillation. 
% The fine-grained classifier is trained with the cross-entropy loss ($L_{CE_{fine}}$), learns information that is sufficient to learn the coarse-classifiers. The other coarse-classifiers are learned mutually 
%, the other coarse-classifiers 
% Instead, we encourage mutual learning between the classifiers at different levels. % the fine-grained and coarse-grained classifier act as a teacher-student mod
% Online Mutual Distillation 
% - online - because teacher and student learning together.. 
% - mutual - teacher learning from student and student learning from teacher. 
% - KD and Re-KD can be said linking with label smooth regularization. 
% - But can we link this to label smoothing regularization? Label regularization in \cite{} revisting knowledge distillation is on offline based learning.. where the entropy of teacher is kept fixed. in online learning, it is not the same case. The formulation of online learning is not yet analyzed separately in the literature.
% - For KD with mutual learning, the distillation loss of two peers is based on the KL divergence..
% - logit distillation
%Instead, we enforce the consistency across classifiers at different levels by using soft labels and a symmetric entropy-based loss function. We minimize the Jensen-Shannon Divergence (JSD) \cite{fuglede_2004_jensen} between the predictions of a coarse classifier $g^{h-1}(\cdot)$ and the soft labels obtained from the next fine-level classifier $g^h(\cdot)$. 
As defined above, for a given class label $A\in\calC^{h-1}$, let $P[\widehat{y}^{h-1}\!=\!A|\bx_i]$ denote the probability of the sample $\bx_i$ belonging to the class $A$, which is computed as 
\begin{gather}
\label{eqn:total_prob}
P\left[\widehat{y}_i^{h-1}\!=\!A|\bx_i\right] = \sum_{k=1}^{|A|} p^h(\widehat{y}_i^h=A_k|\bx_i;\bW^{h})
%p^{(h+1)}(\hat{y_i}=A_1|x_i;\theta_{h+1}) + p^{(h+1)}(\hat{y_i}=A_2|x_i;\theta_{h+1})
\end{gather}
The probabilities $P[c], \forall c\in\calC^{h-1}$ are concatenated together to construct the probability vector $\widehat{p}^{h-1}(\widehat{y}_i^{h-1}|\bx_i)$, which is used as the soft label for $\bx_i$. This soft label generation process is illustrated in Fig. \ref{fig:notations}.

The JSD is minimized between the soft labels and the predictions from the classifier $g^h(\cdot)$. For convenience, we use $p_i^h$ to refer to $ p^h(\hat{y_i}^h|x_i;\bW^h) $ and similarly $\widehat{p}_i^h$ for the corresponding soft label. The JSD based total \JSD is computed by summing the pairwise losses across the levels
\begin{gather}
\text{L}_{shc} = \sum_{h=1}^{H-1}JS^h\left(p_i^h||\widehat{p}_i^h\right) = \frac{1}{2} \sum_{h=1}^{H-1} (\text{KL}(p_i^h || m) + \text{KL}(\widehat{p}_i^h || m))
\label{eqn:shc_loss}
\end{gather}
where $m$ = $\frac{1}{2}(p_i^h + \widehat{p}_i^h)$ and KL$(\cdot||\cdot)$ refers to Kullback-Leibler divergence. 

\begin{wrapfigure}[23]{r}{0.5\textwidth}
  \begin{center}
  \vspace{-5mm}
    \includegraphics[width=0.42\textwidth]{figures/notations.pdf}
      \vspace{-5mm}
  \end{center}
  \caption{Constructing the soft labels for training the coarse-level classifiers. The super-class target probability is the sum of its sub-classes' predicted probability. The colors indicate the class relationships across levels $h-1$ and $h$.}
  \label{fig:notations}
\end{wrapfigure}

It is important to highlight the key difference between the soft labels generated above and those defined in \cite{bertinetto_2020_CVPR}. The latter are designed using the LCA-based distance between classes, whereas our choice of soft labels can be interpreted as a \emph{learned} label-smoothing that better regularizes the coarse-level classifiers. Yuan et al. \cite{Yuan_2020_CVPR} make a similar argument about label smoothing in the context of knowledge distillation. The use of a symmetric loss like in eqn. (\ref{eqn:shc_loss}) further enables the classifiers at both levels to jointly drive the feature space learning. This behavior of the coarse classifiers improving the performance of the finer-level classifiers is analogous to the Reversed Knowledge Distillation (Re-KD) setting as presented in \cite{Yuan_2020_CVPR}, where the authors showed that a student ($g^{h-1}(\cdot)$) is capable of improving the performance of the teacher ($g^h(\cdot)$).  

\subsection{\dissimilar ($L_m$)}
While $\text{L}_{shc}$ improves the mistake severity (as we show in Sec. \ref{sec:analysis}) successfully by virtue of better regularization, it does not directly encourage discrimination between coarse-level classes. Therefore, we use a pairwise margin-based loss to promote a more discriminative feature space. We use this loss over coarser levels $h \in \calH$ where $\calH$ is [$k$, $H-1$] and $k$ ranges from [$1$ , $H-1$]. For a given batch of samples, we create pairs of samples that have dissimilar labels at a level $h$, i.e., $\calB^h = \{(i,j) | y^h_i\neq y^h_j\}$. Then we compute the margin loss over the batch as
\begin{gather}
    L_{m} = \sum_{h\in\calH} \sum_{(i,j)\in\calB^h}\max\left(0, m - \text{JS}^h(p^h_i || p^h_j)\right)
    \label{eqn:margin_loss}
\end{gather}
where $p^h_i$ is the softmax probability generated by $g^h(f_\phi(\bx_i))$ and $m$ is the margin. The margin loss is only applied to the coarser levels of the hierarchy, as the cross-entropy loss of (\ref{eqn:cross-entropy}) is sufficient for fine-grained discrimination. 

%The \dissimilar maximizes the JS divergence between the probability distribution of dissimilar pairs. For a batch of data, we randomly create pairs with different ground-truth labels at every hierarchical level $h$. The \dissimilar at any level $h$ between the distributions $p$ and $q$ of dissimilar pairs is given by:
% The pairwise \dissimilar at any level $h$ is given by: 
% The \dissimilar uses dissimilar pairs at coarser-levels. We maximize the JS Divergence between the probability distribution of dissimilar pairs. The pairwise \dissimilar at any level $h$ is given by: 

% \begin{gather}
%     L_{dsim}^h = max(0, m - \text{JS}^h(p ; q))
% \end{gather}
% where $m$ is the margin and $p$ and $q$ are the probability distributions of dissimilar pairs from classifier at level $h$. 

% The total dissimilar loss $L_{dsim}$ is given by: 
% \begin{gather}
%     L_{tdsim} = \sum_{h=1}^{H-1} L_{dsim}^h
% \end{gather}


\subsection{\weightconst ($L_{gc}$)}
\ours uses classifiers at all the levels of hierarchy. In a hierarchy-aware feature space, the weight vectors of the coarse class and its fine-grained classes should be correlated. The losses introduced in the previous subsections impose probabilistic consistency across the classifier predictions, and only indirectly affect the feature space geometry. In order to better orient the feature space to inherit the label space hierarchy, we use a geometric consistency loss. As before, let $A\in\calC^{h-1}$ be a given super-class and its sub-classes be $A_k\in\calC^h,~k=1,\ldots,|A|$. Let the weight vector corresponding to the super-class $A$ be $\bw^{h-1}_A$ and similarly the weight vectors corresponding to the sub-classes be $\bw^{h}_{A_k}$. Note that the classifier $g^{h-1}(\cdot)$ is defined by the weight matrix $\bW^{h-1}$, which is obtained by stacking the weight vectors $\bw_c,~c\in\calC^{h-1}$. We further constrain each weight vector to be unit norm $||\bw^h_c||_2=1, \forall c,h $, across all classifiers. For the super-class $A\in\calC^{h-1}$, we define the target weight vector as $\widehat{\bw}_A^{h-1} = \widetilde{\bw}^{h-1}_A/||\widetilde{\bw}_A^{h-1}||_2$, where $\widetilde{\bw}_A^{h-1}=\sum_{k=1}^{|A|}\bw_{A_k}^h$. Thus, the \weightconst loss to be minimized is 
\begin{gather}
    L_{gc} = \sum_{h=1}^{H-1} \sum_{c\in\calC^h}\left(1 - \cos\left(\bw_c^{h},\widehat{\bw}_c^h\right)\right)
    \label{eqn:gc_loss}
\end{gather}
where $\cos\left(\bw_c^{h},\widehat{\bw}_c^h\right)$ refers to the cosine similarity between the weight vectors $\bw_c^{h}$ and $\widehat{\bw}_c^h$.
% Our geometric consistency loss explicitly imposes high angular similarity between the classifier weights corresponding to the super-class and its sub-classes. This loss subsequently promotes the feature space distribution of all sub-classes to be more correlated than the other classes, thereby reducing the chance of making a more severe misclassification. Unsurprisingly, we observe in our experiments that adding this geometric consistency loss further reduces mistake severity, without significantly impacting the top-$1$ error. 

% We denote the weight vector of coarse class $C$ at level $h$ by $W_C^{h}$. We fix the weights $||W_C^h||=1$ of every class across all the levels. Note that the logit is $W_C^h . x_i$=$||W_C^h|| ||x_i|| cos\theta_C^h$. The normalization step across all the levels of the classifier force the predictions to depend only on the angle between the weight vector and the feature ($||x_i||$ is same across all the levels of the hierarchy). 
% To further constraint these weight vectors to hold the relationship in the label hierarchy, we fix the weights $||W_j||=1$ of every class across all the levels
%The weight vectors of different classifiers learned in a hierarchy-aware feature space should be aligned. The weight vector of coarse class should be aligned with the linear combination of the weight vectors of its fine-grained classes. We first normalize the weight vectors of all the classes across all the classifiers before applying softmax at the output. For a category $C$ at any level $h$, the l2-normalized weight is given by:  
%  \begin{gather}
%     W_C^h = \frac{W_C^h}{||W_C^h||_2}
% \end{gather}
% We re-normalize all the weight vectors to lie on a normalized hypersphere, 
% Adding weight constraints: \\
%     First L2-Normalize weights:
   
    % Softmax Loss: 
    % \begin{gather}
    %     \text{minimize} \frac{-1}{M} \sum_{i=1}^{N}\text{log} (\frac{{e^{W_{ci}^{h^T}} f(xi) + b_{ci}^h}}{\sum_{j=1}^{C} e^{W_{ci}^{h^T} f(xi) + b_{ci}^h}})
    % \end{gather}
    % Again L2-normalize weights;
    % \begin{gather}
    %     W_c^h = \frac{W_c^h}{||W_c^h||_2}
    % \end{gather}
    % Convex combination (summation) of weights of sub-classes of a super-class (L2-normalized vectors) should be aligned to L2-normalized weight vector of that coarse class. 
% On a normalized hypersphere, the weight vector of coarse class should be aligned with the linear combination of the weight vectors of its fine-grained classes. %We denote the weight vector of coarse class $C$ at level $h-1$ by $W_C^{h-1}$. 
% Let $c$ $\in [1, K]$ represents indices of the sub-classes at level $h$ belonging to the coarse-class $C$ at level $h-1$. We hypothesize that the convex combination of weight vectors of sub-classes of a super-class should be aligned with the weight vector of its coarse class. For simplicity, we use the summation of the sub-classes' weight vectors to represent the super-class's weight vector. The approximated weight vector using summation is thus given by:
% \begin{gather}
%     \hat{W}_C^{h-1} = \sum_{c=1}^{K}W_c^h
% \end{gather}
% To align the weights of super-class with it's sub-classes, we maximize the cosine similarity between $W_C^{h-1}$ and $\hat{W_C^{h-1}}$.
% \begin{gather}
%   L_{sim}^{h-1} = \text{cos}(W_C^{h-1}, \hat{W}_C^{h-1})
% \end{gather}
% Similar to \JSD, we calculate $L_{sim}$ loss pairwise across all the levels. The total \weightconst is given by: 

% \begin{gather}
% L_{tsim} = \sum_{h=1}^{H-1}L_{sim}^h   % {\text{JS}}^h
% \end{gather}

Finally, the total loss is given by $L_{total} =$  \CEfinestsymb + \JSDsymb + \dissimilarsymb + \weightconstsymb .

% Let $H$ be the number of hierarchical levels, $K^i$ be the number of classes at the $i$-th level of the hierarchy, where $i=1$ corresponds to coarsest and $i=H$ is the finest-level. Let $\cal{F}(.)$ be the feature extractor and ${\cal{G}}^1(.)$, ${\cal{G}}^2(.)$, ${\cal{G}}^3(.)$ $\ldots$ ${\cal{G}}^H(.)$ be different hierarchical classifiers. 

% Let $\cal{X}$ = $\{ x_i, y_i^h \}$ be the set of images and their labels at level $h$ where $h$ $\in$ [$1, 2, \ldots H$]. Let $p^h(\hat{y_i}|x_i;\theta)$ = ${\cal{G}}^h(F(x_i))$ refers to the predicted probability of image $x_i$ from the model $\theta$ from $h$-level hierarchical classifier. 

%To model the hierarchies in the data, mixture distributions can be one of the possible ways. The finest level of the hierarchy can be considered to be the distribution of the fine-grained classes. Semantically similar classes should follow similar data distribution and therefore, higher levels of hierarchy can be composite of mixture distributions of semantically similar classes. For a super-class $C$ at level $h$ and its sub-classes $c \in C$ at level $h+1$.

% \begin{comment}
% \begin{gather}
% p^h(\hat{y_i}=C|x_i;\theta) = \sum_{c \in C} \pi_i   p^{h+1}(\hat{y_i}=c|x_i;\theta)
% \end{gather}
% where $\Pi_i$ represents the mixing weights. Can be a uniform distribution, or, ... 
% \end{comment}


==> alldefin.tex <==
%%%%%%%%  page layout

%\textheight = 8in
%\textwidth = 4.7in
%\evensidemargin= 0.0in
%\oddsidemargin= 0.0in
%\topmargin = - 0.5in
%\headsep = 0.5in
%\columnsep = 0.2in
%\headheight = 0.0in
%\parskip = .1in
%\parindent = 0.4in
\RequirePackage{xspace}

\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{c.f}\onedot} \def\Cf{\emph{C.f}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}
\makeatother


\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbQ}{\mathbb{Q}}

\newcommand{\GL}[1]{\mbox{$\mathbf{GL}(#1)$}}
\newcommand{\SL}[1]{\mbox{$\mathbf{SL}(#1)$}}
\newcommand{\SE}[1]{\mbox{$\mathbf{SE}(#1)$}}
\newcommand{\se}[1]{\mbox{\tengoth{se}(#1)}}
\newcommand{\SO}[1]{\mbox{$\mathbf{SO}(#1)$}}
% \newcommand{\so}[1]{\mbox{\tengoth{so}(#1)}}
\newcommand{\Af}[1]{\mbox{$\mathbf{A}(#1)$}}
\newcommand{\Grass}[2]{\mathbf{G}_{#1,#2}}
\newcommand{\Sym}[1]{Sym_{#1}^{+}}

\newcommand{\X}{\mbox{$\bf X$}}

\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calH}{\mathcal{H}}


\newcommand{\Tan}[2]{T_{#1}(#2)}
\newcommand{\func}[1]{\mathfrak{F}(#1)}
\newcommand{\vecf}[1]{\mathfrak{X}(#1)}



\newcommand{\SSS}{\scriptscriptstyle}
\newcommand{\vc}[1]{\mbox{\boldmath ${#1}$}}

%%%%%%%%%%%mine%%%%%%%%%%%%%%%%%%%%
\newcommand{\eye}[1]{\mbox{\boldmath $\bf{e}_{#1}$}}
\newcommand{\zio}{\vc{z}_{io}}
\newcommand{\zi}{\vc{z}_{i}}
\newcommand{\zihat}{\hat{\vc{z}}_{i}}
\newcommand{\zicheck}{\check{\vc{z}}_{i}}
\newcommand{\zj}{\vc{z}_{j}}
\newcommand{\zjhat}{\hat{\vc{z}}_{j}}
\newcommand{\zjcheck}{\check{\vc{z}}_{j}}
\newcommand{\ro}{\vc{r}_{o}}
\newcommand{\rr}{\vc{r}}
\newcommand{\rhat}{\hat{\vc{r}}}
\newcommand{\rcheck}{\check{\vc{r}}}
\newcommand{\tv}{\vc{t}}
\newcommand{\that}{\hat{\vc{t}}}
\newcommand{\Covmat}{\vc{C}}
\newcommand{\bvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\mydef}{\stackrel{\Delta}{=}}
\newcommand{\f}{\mbox{$\vc f$}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ftilde}{\tilde{f}}

%\renewcommand{\labelitemi}{} %{--}
\newfont{\tengoth}{eufm10}
\newcommand{\lieg}{\mbox{\tengoth{g}}}
\newcommand{\lieh}{\mbox{\tengoth{h}}}

\newcommand{\luv}{$\rm \  L^{*}u^{*}v^{*} \  $}
\newcommand{\lab}{$\rm \  L^{*}a^{*}b^{*} \  $}

\newcommand{\trans}{^{\top}}

\newcommand{\myrfe}[1]{(\ref{eqn:#1})}
\newcommand{\myrff}[1]{\ref{fig:#1}}
\newcommand{\myrfs}[1]{\ref{sec:#1}}
\newcommand{\myrft}[1]{\ref{tab:#1}}

\newcommand{\bphi}{\mbox{\boldmath $\phi$}}
\newcommand{\bPhi}{\mbox{\boldmath $\Phi$}}
\newcommand{\blambda}{\mbox{\boldmath $\lambda$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\balpha}{\mbox{\boldmath $\alpha$}}
\newcommand{\balphahat}{\mbox{\boldmath $\hat{\alpha}$}}
\newcommand{\alphahat}{\mbox{$\hat{\alpha}$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bsigma}{\mbox{\boldmath $\sigma$}}
\newcommand{\bSigmahat}{\mbox{\boldmath $\hat{\Sigma}$}}
\newcommand{\boldeta}{\mbox{\boldmath $\eta$}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bxi}{\mbox{\boldmath $\xi$}}
\newcommand{\bthetahat}{\mbox{\boldmath $\hat{\theta}$}}
\newcommand{\bthetacheck}{\mbox{\boldmath $\check{\theta}$}}
\newcommand{\bthetahathat}{\mbox{\boldmath $\hat{\hat{\theta}}$}}
\newcommand{\bthetabar}{\mbox{\boldmath $\bar{\theta}$}}
\newcommand{\bTheta}{\mbox{\boldmath $\Theta$}}
\newcommand{\bThetahat}{\mbox{\boldmath $\hat{\Theta}$}}
\newcommand{\bldomega}{\mbox{\boldmath $\omega$}}
\newcommand{\boldpi}{\mbox{\boldmath $\pi$}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bbetahat}{\mbox{\boldmath $\hat{\beta}$}}
\newcommand{\bPsi}{\mbox{\boldmath $\Psi$}}
\newcommand{\bGamma}{\mbox{\boldmath $\Gamma$}}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bnu}{\mbox{\boldmath $\nu$}}
\newcommand{\btau}{\mbox{\boldmath $\tau$}}
\newcommand{\talpha}{\tilde\alpha}
\newcommand{\tgamma}{\tilde\gamma}
\newcommand{\teta}{\tilde\eta}

\newcommand{\bomega}{\mbox{\boldmath $\omega$}}
\newcommand{\vomega}{\vc{\omega}}

\newcommand{\vyhat}{\hat{\vc{y}}}
\newcommand{\x}{\vc{x}}
\newcommand{\y}{\vc{y}}
\newcommand{\ty}{\tilde\y}
\newcommand{\tbC}{\tilde{\bf C}}

\newcommand{\tbx}{\tilde{\vc{x}}}
\newcommand{\tbX}{\tilde{\vc{X}}}
\newcommand{\bl}{\mbox{$\mathbf{l}$}}
\newcommand{\tbe}{\tilde{\vc{e}}}
\newcommand{\bi}{{\vc{i}}}


\newcommand{\be}{\mbox{$\mathbf{e}$}}
\newcommand{\bx}{\mbox{$\mathbf{x}$}}
\newcommand{\by}{\mbox{$\bf y$}}
\newcommand{\bz}{\mbox{$\bf z$}}
\newcommand{\bxs}{\mbox{$\bf\scriptstyle x$}}
\newcommand{\bzs}{\mbox{$\bf\scriptstyle z$}}
\newcommand{\bys}{\mbox{$\bf\scriptstyle y$}}
\newcommand{\bzhat}{\mbox{$\hat{\bf z}$}}
\newcommand{\bp}{\mbox{$\bf p$}}
\newcommand{\bq}{\mbox{$\bf q$}}
\newcommand{\bs}{\mbox{$\bf s$}}
\newcommand{\bn}{\mbox{$\bf n$}}
\newcommand{\bh}{\mbox{$\bf h$}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\bm}{\mbox{$\bf m$}}
\newcommand{\bu}{\mbox{$\bf u$}}
\newcommand{\bv}{\mbox{$\bf v$}}
\newcommand{\bw}{\mbox{$\bf w$}}
\newcommand{\bc}{\mbox{$\bf c$}}
\newcommand{\bg}{\mbox{$\bf g$}}

\newcommand{\bA}{\mbox{$\bf A$}}
\newcommand{\bB}{\mbox{$\bf B$}}
\newcommand{\bC}{\mbox{$\bf C$}}
\newcommand{\bD}{\mbox{$\bf D$}}
\newcommand{\bE}{\mbox{$\bf E$}}
\newcommand{\bF}{\mbox{$\bf F$}}
\newcommand{\bG}{\mbox{$\bf G$}}
\newcommand{\bH}{\mbox{$\bf H$}}
\newcommand{\bI}{\mbox{$\bf I$}}
\newcommand{\bJ}{\mbox{$\bf J$}}
\newcommand{\bK}{\mbox{$\bf K$}}
\newcommand{\bM}{\mbox{$\bf M$}}
\newcommand{\bL}{\mbox{$\bf L$}}
\newcommand{\bN}{\mbox{$\bf N$}}
\newcommand{\bP}{\mbox{$\bf P$}}
\newcommand{\bQ}{\mbox{$\bf Q$}}
\newcommand{\bO}{\mbox{$\bf O$}}
\newcommand{\bR}{\mbox{$\bf R$}}
\newcommand{\bS}{\mbox{$\bf S$}}
\newcommand{\bT}{\mbox{$\bf T$}}
\newcommand{\bU}{\mbox{$\bf U$}}
\newcommand{\bV}{\mbox{$\bf V$}}
\newcommand{\bW}{\mbox{$\bf W$}}
\newcommand{\bX}{\mbox{$\bf X$}}
\newcommand{\bY}{\mbox{$\bf Y$}}
\newcommand{\bZ}{\mbox{$\bf Z$}}




\newcommand{\vecy}{{\vc{y}}}
\newcommand{\tH}{\widetilde{{\bf H}}}

\newcommand{\px}{\mbox{$p(\x)$}}
\newcommand{\py}{\mbox{$p(\y)$}}

\newcommand{\exi}{\mbox{exp}\left(-\left\|\frac{\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxz}{\mbox{exp}\left(-\left\|\frac{\y_j-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxo}{\mbox{exp}\left(-\left\|\frac{\y_{j+1}-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\ey}{\mbox{exp}\left(\left\|\frac{\y_{j+1}}{\displaystyle{h}}\right\|^2\right)}

%%%%%%%%%%%%%%%%%%%%%% Kernel Density Stuff %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\myK}{K\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}
\newcommand{\myKy}{K\left(\frac{\y^j-\x_{i}}{\displaystyle{h}}\right)}

\newcommand{\myG}{G\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}

\newcommand{\myk}{k\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\myky}{k\left(\left\|\frac{\y^j-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\myki}{k\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}
\newcommand{\mykyi}{k\left(\left\|\frac{\y^j-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}

\newcommand{\myg}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\mygy}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\mygi}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}
\newcommand{\mygyi}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}_i}\right\|^2\right)}

\newcommand{\mygd}{g\left(d^2(\mathbf{x},\mathbf{x}_i)/h^2\right)}

\newcommand{\MSE}{\mbox{MSE}}
\newcommand{\MISE}{\mbox{MISE}}



\newcommand{\lsup}[2]{\ensuremath{{}^{#1}\!{#2}}}
\newcommand{\hbo}[1]{\hat{{\bf #1}}}

%%%%%%%%  operators
\newcommand{\med}[1]{\mathop{\mbox{med}}\limits_{#1}}
\newcommand{\var}{\mbox{var}}
\newcommand{\bias}{\mbox{bias}}
\newcommand{\diag}{\mbox{\bf diag}}
\newcommand{\mytr}[1]{{\rm trace} [ #1 ]}
\newcommand{\mymax}[1]{\mathop{\mbox{max}}\limits_{#1}}
\newcommand{\mydet}[1]{{\rm det} [ #1 ]}
\newcommand{\vect}{\mbox{\bf vec}}

\newcommand{\myexps}{\mbox{exp}\left(-\frac{1}{2}\|\x\|^2\right)}
\newcommand{\maha}{{\rm D}\left[\x, \x_i, \bH\right]^2}
\newcommand{\mahai}{{\rm D}\left[\x, \x_i, \bH_i\right]^2}
\newcommand{\myexpm}{\mbox{exp}\left(-\frac{1}{2}\maha\right)}
\newcommand{\myexpmi}{\mbox{exp}\left(-\frac{1}{2}\mahai\right)}

\newcommand{\tr}{\mbox{tr\ }}



\newcommand{\myave}[1]{\mathop{\mbox{ave}}\limits_{#1}}

\newcommand{\ww}{{\vc{w}}}
\newcommand{\tbY}{\tilde\Y}

\newcommand{\bb}{\vc{b}}

\newcommand{\Jc}{\mathcal{J}}
\newcommand{\bzeta}{\vc{\zeta}}

